Robust Temporally Coherent Laplacian Protrusion Segmentation of 3D Articulated Bodies

In motion analysis and understanding it is important to be able to fit a suitable model or structure to the temporal series of observed data, in order to describe motion patterns in a compact way, and to discriminate between them. In an unsupervised context, i.e., no prior model of the moving object(s) is available, such a structure has to be learned from the data in a bottom-up fashion. In recent times, volumetric approaches in which the motion is captured from a number of cameras and a voxel-set representation of the body is built from the camera views, have gained ground due to attractive features such as inherent view-invariance and robustness to occlusions. Automatic, unsupervised segmentation of moving bodies along entire sequences, in a temporally-coherent and robust way, has the potential to provide a means of constructing a bottom-up model of the moving body, and track motion cues that may be later exploited for motion classification. Spectral methods such as locally linear embedding (LLE) can be useful in this context, as they preserve "protrusions", i.e., high-curvature regions of the 3D volume, of articulated shapes, while improving their separation in a lower dimensional space, making them in this way easier to cluster. In this paper we therefore propose a spectral approach to unsupervised and temporally-coherent body-protrusion segmentation along time sequences. Volumetric shapes are clustered in an embedding space, clusters are propagated in time to ensure coherence, and merged or split to accommodate changes in the body's topology. Experiments on both synthetic and real sequences of dense voxel-set data are shown. This supports the ability of the proposed method to cluster body-parts consistently over time in a totally unsupervised fashion, its robustness to sampling density and shape quality, and its potential for bottom-up model construction

==> CoverLetter-R1.tex <==
\pagestyle{empty}
\onecolumn
\begin{center} 
Response to Reviews \vspace{0.5cm}\\
{\Large ``Robust temporally coherent Laplacian protrusion segmentation of 3D articulated bodies''}\vspace{0.5cm}\\
submission reference: \#VISI-D-12-02620
\end{center}

\vspace{0.5cm}
\noindent
\textbf{Editor's comments and recommendation:}\\

We have received two reviews for your manuscript.  Unfortunately several other reviewers did not respond despite their acceptance to review.  Nevertheless, I went through the two reviews and the manuscript and came to the conclusion that your manuscript can be accepted after a minor revision.\\

One reviewer points out missing self-citations and lack of novelty.  Since these missing citations are all workshop or conference papers, I believe that this is no reason for rejection.  Nevertheless, I recommend to include these citations and to possibly clarify what is novel with respect to these conference papers - even if the journal paper just summarizes the results reported in the various workshops and conferences, I believe that is a sufficient contribution.  But it is indeed the authors' job to clarify this precisely.  I also believe that the proposed 3D segmentation of reconstructed objects is a core computer vision challenge and by no means out of scope.  Please also include the suggestions for improvement done by the second reviewer.  Congratulations on your paper being finally accepted!
\\

\noindent
\textbf{Authors' answer:}\\

We thank the reviewers for taking the time to review our submission. Based on their comments and on the Editor's recommendation, we prepared a revised version of our paper.

Please find below detailed answers to the reviewers' questions. The changes made to the paper can be easily tracked by clicking on the links incorporated in our answers, e.g., \refcm{self-citations}.


\begin{answerreviewer}[The manuscript describes a method for segmenting 3D articulated bodies coherently over time.]
 \qa{By cross-reading previous works of the same authors [50], [67-71], I have got the impression that the presented manuscript is
a mixture and mainly a copy of these works. More importantly, I cannot see any novelties over these works.
It is the task of the authors explicitly state novelties and contributions over existing work which has not been done in the presented manuscript.
Moreover, except of [50], none of the previous works have been cited, which I consider as self-plagiarism.
The contribution of the manuscript is completely unclear.
}{The authors took these criticisms seriously and revised the manuscript such as to incorporate self-citations and to clarify the contribution of the manuscript. Please refer to our detailed answers below.}

\qa{- missing references:

[67] Fabio Cuzzolin, Diana Mateus, Edmond Boyer, and Radu Horaud
Robust spectral 3D-bodypart segmentation in time
in "Human Motion - Understanding, Modeling, Capture and Animation",
Lecture Notes in Computer Science, Vol. 4814/2007, pages 196-211
Seidel, H.-P.; Wang, Y.; Rosenhahn, B.; Mori, G. (Eds.)
Springer Berlin / Heidelberg, 2007

[68] Diana Mateus, Fabio Cuzzolin, Radu P. Horaud, Edmond Boyer.
Articulated Shape Matching by Robust Alignment of Embedded Representations.
IEEE Workshop on 3D Representation for Recognition (3DRR 2007) - October 2007

[69] Diana Mateus, Fabio Cuzzolin, Edmond Boyer, and Radu Horaud
Articulated Shape Matching Using Locally Linear Embedding and Orthogonal Alignment
IEEE International Conference on Computer Vision (ICCV'07) - NTRL Workshop
Rio de Janeiro, October 2007

[70] Fabio Cuzzolin, Diana Mateus, David Knossow, Edmond Boyer, Radu P. Horaud.
Coherent Laplacian 3-D Protrusion Segmentation.
Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition - CVPR 2008

[71] Diana Mateus
Spectral Tools for Unsupervised Modeling of Articulated Objects from Multiple-view Videos.
PhD Thesis, INRIA Grenoble (Institut National de Recherche en Informatique et Automatique) and
Institute National Polythechnique de Grenoble (INPG). September 2009.
}
{The manuscript is indeed an extended version of a workshop paper, Cuzzolin et al. 2007 (or [67]) and a CVPR paper, Cuzzolin at al. 2008 (or [70]). The other two papers mentioned by the reviewer ([68] and [69]) deal with articulated shape matching and not with articulated shape segmentation over time, hence they need not be cited here. These two aspects (matching and segmentation) are addressed completely differently in [67,70] (segmentation) and [68,69] (matching), they only share the authors. The final citation  ([71]) is the PhD dissertation of one of the three authors of the current submission. }

\qa{The presented manuscript uses numerous results, whole text sections and e.g. all 11 figures from [67].
Section 3 is almost entirely copied from [67]. The algorithm description in 3.4 and 3.5 can also been found in [70,71].
Section 4.6.2 mainly repeats the content of [Section 2, 70].
Almost every figure and all experiments in the manuscript can be found in one or several of the works [67-71].
Without any citation to these works the manuscript can be considered as self-plagiarism.
Moreover, the novelties and contributions of the presented manuscript over previous work by the authors are not mentioned and remain unclear.}
{We incorporated a paragraph (see \refcm{self-citations}) that cites [67,70] (Cuzzolin et al. 2007 and Cuzzolin et al. 2008) and that explains the extensions and the novel material to be found in the current manuscript. [71] is a PhD manuscript and it is common practice to reproduce some of the thesis results in a journal submission.}

\qa{Reference [5] is the same as [4]}{Corrected}

\qa{Page 2, Line 18: references [30] and [36] are not appropriate, because they only consider 3d reconstruction of static scenes.
  "capturing of motion" is not considered in these works.}{We modified the paragraph to make a clearer distinction between methods that just perform reconstruction and methods that perform both reconstruction and motion capture, please see \refcm{capture}.}
\end{answerreviewer}

\stepcounter{reviewer}

\begin{answerreviewer}[The paper proposes a method for the segmentation of protruding parts in 4D data sets capturing articulated body structures reconstructed from multiple synchronized video streams.]
%\typo{P2L13: "its face" $\rightarrow$ "his/her face"}{Done.}
\qa{The paper is well-written and the single steps of the proposed approach are convincingly motivated with numerous examples. Also, the experimental evaluation of the approach is exhaustive and contains qualitative as well as quantitative evaluation on synthetic and real-world data. Moreover, the effect of the single parameters on the performance of the algorithm are explored and demonstrated. Unfortunately, I am not an expert in clustering and for me it is difficult to judge the novelty of the technique or the relevance of the demonstrated comparisons to the time-consistent EM clustering and ISOMAP clustering. Nevertheless, I could state that the method seems plausible and technically sound to me.}{In terms of clustering, there are two main possibilities: clustering in the initial 3D space, or clustering in the embedded or spectral space. We opted to compare our results to two widely used methods.}
\qa{One important question to address is also the suitability of the paper for this journal. Actually, the link to computer vision is only indirect as the authors assume the reconstructed models as given.}{We believe that 3D model segmentation is a computer vision problem. In particular we address the issue of coherent segmentation over time -- this problem is typically encountered with data coming from visual sensors and, therefore, processing this type of data in order to robustly extract compact and higher-level representations, is a computer vision problem.}
\qa{Section 1.1. should focus on the novelty only. The citation of relevant papers should be shifted to the previous paragraph. Also, terms like "stereo-reconstructed voxels" should be avoided as they are not very clear. Use for example "stereo-based volumetric reconstruction" instead.}{We removed citations from this section and corrected the terms as suggested by the reviewer.}
\qa{The renderings used throughout the paper should be explained. Obviously, the volumetric reconstructions are converted into point clouds but this step should be elucidated.}{We added a sentence (see \refcm{point-cloud}) stating that voxel representations are visualized as point clouds.}
\qa{The bullet points in Section 2.1. are not consistent since some of them are just headwords and others are full sentences}{Corrected}
\qa{Fig. 3 is not very clear to me. Why is LLE space 3D and ISOMAP space 2D? Is d=3 in both cases?}{In both cases the embedding is with d=3.}
\qa{Fig. 12 and 13 are also a little bit confusing. Why are the black lines (which represent the ground truth) not the same? Is it possible to compare the LLE-based approach and the time-consistent EM clustering directly in a single plot for each sequence?}{The reason is, since segmentation is ambiguous (arms as a whole or split at the elbow), we compute the score for \textbf{three different ground truth segmentations} (also illustrated in Figure~\ref{fig:ground} - right)}


\qa{The second application demonstrated in Section 5 is not very convincing. For an augmented reality application one doesn't need to fit blobs in order to realize the interaction with a virtual environment. In fact, a volumetric model already provides implicit information about the space occupancy which can efficiently be used for collision detection and interaction with the environment.}{Indeed. The idea here was to do bottom up motion capture, i.e., to identify the rigid links composing the body in an unsupervised way. The proposed representation based on ellipsoids leads to an implicit surface representation which has also been widely used in interactive graphics applications. We added a phrase to make this point clear, please see \refcm{virtual}.}
\end{answerreviewer}

\clearpage
\pagestyle{plain}
\setcounter{page}{1}
